Multi-task Reinforcement Learning in Reproducing Kernel Hilbert Spaces via Cross-learning

Reinforcement learning (RL) is a framework to optimize a control policy using rewards that are revealed by the system as a response to a control action. In its standard form, RL involves a single agent that uses its policy to accomplish a specific task. These methods require large amounts of reward samples to achieve good performance, and may not generalize well when the task is modified, even if the new task is related. In this paper we are interested in a collaborative scheme in which multiple agents with different tasks optimize their policies jointly. To this end, we introduce cross-learning, in which agents tackling related tasks have their policies constrained to be close to one another. Two properties make our new approach attractive: (i) it produces a multi-task central policy that can be used as a starting point to adapt quickly to one of the tasks trained for, in a situation when the agent does not know which task is currently facing, and (ii) as in meta-learning, it adapts to environments related but different to those seen during training. We focus on continuous policies belonging to reproducing kernel Hilbert spaces for which we bound the distance between the task-specific policies and the cross-learned policy. To solve the resulting optimization problem, we resort to a projected policy gradient algorithm and prove that it converges to a near-optimal solution with high probability. We evaluate our methodology with a navigation example in which agents can move through environments with obstacles of multiple shapes and avoid obstacles not trained for.

==> fig/fig_projection.tex <==
\begin{tikzpicture}
	\pgfplotsset{grid style={dashed,gray!50}}
	\begin{axis}[
		%minor tick num=1,
		%xlabel={$x$},
		%ylabel={$y$},
		%ylabel near ticks,
		ticks=none,
		grid=none,
		axis line style={draw=none},
            	%xticklabel style = {font=\small},
            	%yticklabel style = {font=\small},
           	width=\columnwidth, 
		height=0.86\columnwidth, 
		xmin=-3,xmax=11,ymin=-3,ymax=9
	]
	\addplot [only marks,mark=o,mark size=3pt,mark options={black,solid}]
		table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataPoints.dat};
	\addplot [only marks,mark=*,mark size=3pt,mark options={red,solid}]
		table[x index=2,y index=3, col sep=comma]{fig/projection_data/dataPoints.dat};
	\addplot [only marks,mark=*,mark size=3pt,mark options={red,solid,fill=white}]
		table[x index=1,y index=2, col sep=comma]{fig/projection_data/dataPointsCenters.dat};
			
	\addplot [color=red,dashed,mark=none]
		table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataLine1.dat};
	\addplot [color=red,dashed,mark=none]
		table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataLine2.dat};
	\addplot [color=red,dashed,mark=none]
		table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataLine3.dat};			
	\addplot [color=red,dashed,mark=none]
		table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataLine4.dat};
	\addplot [color=red,dashed,mark=none]
		table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataLine5.dat};
	\addplot [color=red,dashed,mark=none]
		table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataLine6.dat};

	\draw[fill=gray!20] (axis cs:5.1868,4.2128) ellipse [x radius=2*1.2*10, y radius=2*1.2*10*10];

	\draw[black,-] (axis cs:5.1868,4.2128) -- (axis cs:5.825,6.525) ;
	\node[] at (axis cs:5.3,5.5) {\small \textcolor{black}{$\epsilon$}};

	\node[] at (axis cs:5.75,4) {\small \textcolor{red}{$g$}};
	\node[] at (axis cs:10.75,8) {\small $\bar{h}_i$};
	\node[] at (axis cs:7.25,6.25) {\small \textcolor{red}{$h_i$}};

	\end{axis}
\end{tikzpicture}



==> fig/fig_projection_relaxed.tex <==
\begin{tikzpicture}
	\pgfplotsset{grid style={dashed,gray!50}}
	\begin{axis}[
		%minor tick num=1,
		%xlabel={$x$},
		%ylabel={$y$},
		%ylabel near ticks,
		%xticklabel style = {font=\small},
		%yticklabel style = {font=\small},
		ticks=none,
		grid=none,
		axis line style={draw=none},
		width=\columnwidth, 
		height=0.86\columnwidth, 
		xmin=-3,xmax=11,ymin=-3,ymax=9
	]
	\addplot [only marks,mark=o,mark size=3pt,mark options={black,solid}]
	table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataPoints.dat};
	\addplot [only marks,mark=*,mark size=3pt,mark options={red,solid}]
	table[x index=2,y index=3, col sep=comma]{fig/projection_data/dataPoints.dat};
	\addplot [only marks,mark=*,mark size=3pt,mark options={blue,solid}]
	table[x index=4,y index=5, col sep=comma]{fig/projection_data/dataPoints.dat};
	\addplot [only marks,mark=*,mark size=3pt,mark options={red,solid,fill=white}]
	table[x index=1,y index=2, col sep=comma]{fig/projection_data/dataPointsCenters.dat};
	\addplot [only marks,mark=*,mark size=3pt,mark options={blue,solid,fill=white}]
	table[x index=3,y index=4, col sep=comma]{fig/projection_data/dataPointsCenters.dat};
	
	\addplot [color=red,dashed,mark=none]
	table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataLine1.dat};
	\addplot [color=red,dashed,mark=none]
	table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataLine2.dat};
	\addplot [color=red,dashed,mark=none]
	table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataLine3.dat};			
	\addplot [color=red,dashed,mark=none]
	table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataLine4.dat};
	\addplot [color=red,dashed,mark=none]
	table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataLine5.dat};
	\addplot [color=red,dashed,mark=none]
	table[x index=0,y index=1, col sep=comma]{fig/projection_data/dataLine6.dat};
	
	\addplot [color=blue,dashed,mark=none]
	table[x index=2,y index=3, col sep=comma]{fig/projection_data/dataLine1.dat};
	\addplot [color=blue,dashed,mark=none]
	table[x index=2,y index=3, col sep=comma]{fig/projection_data/dataLine2.dat};
	\addplot [color=blue,dashed,mark=none]
	table[x index=2,y index=3, col sep=comma]{fig/projection_data/dataLine3.dat};			
	\addplot [color=blue,dashed,mark=none]
	table[x index=2,y index=3, col sep=comma]{fig/projection_data/dataLine4.dat};
	\addplot [color=blue,dashed,mark=none]
	table[x index=2,y index=3, col sep=comma]{fig/projection_data/dataLine5.dat};
	\addplot [color=blue,dashed,mark=none]
	table[x index=2,y index=3, col sep=comma]{fig/projection_data/dataLine6.dat};
	
	\draw[fill=gray!20] (axis cs:5.1868,4.2128) ellipse [x radius=2*1.2*10, y radius=2*1.2*10*10];
	
	\draw[black,-] (axis cs:5.1868,4.2128) -- (axis cs:5.825,6.525) ;
	\node[] at (axis cs:5.3,5.5) {\small \textcolor{black}{$\epsilon$}};
	
	\node[] at (axis cs:5.75,4) {\small \textcolor{red}{$g$}};
	\node[] at (axis cs:5,3.5) {\small \textcolor{blue}{$g$}};
	
	\node[] at (axis cs:5.4,-2) {\small $\bar{h}_i$};
	\node[] at (axis cs:5,1) {\small \textcolor{blue}{$h_i$}};
	\node[] at (axis cs:4.8,2.25) {\small \textcolor{red}{$h_i$}};
	
	\end{axis}
\end{tikzpicture}

==> fig/fig_robot_model.tex <==
\begin{tikzpicture}[scale=1.1,domain=-0.1:10]    

    \node [below] at (0,-1) {Goal};
    \fill[rounded corners,draw=black,fill=black!75] (4,2) -- (5.73,3) -- (5.23,3.86) -- (3.5,2.86) --  cycle;
    \fill[draw=black!50,thick, fill=gray!50] (3,0) circle (1);
    \fill[fill=red] (0,-1) circle (0.05); 
    \draw[dashed] (3.75,2.43) --(2.23,0.64) ; %left intersection
    \draw[dashed] (3.75,2.43) --(3.99,0.1) ;%right intersection
    %Arcs
    % the z line y0=0.578*x0+0.312
    
	\draw[dashed,->] (0.5,0.601) arc (-150:-140:3.72);

	\draw[dashed,->] (1.5,1.165) arc (-150:-137:2.57);
	\draw[dashed,->] (3,2.01) arc (-150:-114:1.05);
	\draw[dashed,<->] (2.6,1.07) arc (-130:-98:2.69);
	\node [below] at (3,-1.1) {Obstacle};
	\node [below] at (0.6,0.3) {$\dot \psi$};	
	\node [below] at (1.5,1.165) {$\phi_g$};		
	\node [below] at (3,2.01) {$\phi_o$};	
	\node [below] at (3.35,0.65) {$\phi_{obs}$};				
	
    \draw[red,->] (3.75,2.43) -- (0,-1) node[right] {$d_g$};
    \draw[red,->] (3.75,2.43) -- (3.3,0.96) node[right] {$d_o$};
    \draw[dashed,->] (3.75,2.43) -- (0,0.312) node[left] {$\dot z$};	
	
\end{tikzpicture}


==> fig/fig_triangle.tex <==
\begin{tikzpicture}[scale = 1]

	\draw[semithick,-] (0,0) -- (5,0) ;
	\draw[semithick,-] (5,0) -- (5,5) ;
	\draw[semithick,-] (0,0) -- (5,5) ;

	% N \epsilon
	\draw[semithick,red,-] (3,0) -- (3,3) ;

	% Line 1
	\draw[semithick,blue,-] (0,0) -- (3,1) ;
	\draw[semithick,red,-] (3,1) -- (5,1.66) ;

	% Line 2
	\draw[semithick,blue,-] (0,0) -- (3,2) ;
	\draw[semithick,red,-] (3,2) -- (5,3.33) ;

	\node at (3,0) [anchor=north] {\footnotesize $N\epsilon^2$};
			
	\draw[decoration={brace, mirror, raise=13}, decorate,semithick,-] (0,0) -- (5,0) node [pos=0.5,anchor=north,yshift=-14] {\footnotesize $b$};

	%\draw[decoration={brace, mirror, raise=13}, decorate,semithick,-] (5,0) -- (5,5) node [pos=0.5,anchor=west,xshift=14] {\footnotesize $a$};
					
	%\node at (3,1) [anchor=north west] {\footnotesize $x_1^2$};
	%\node at (5,1.66) [anchor=north west] {\footnotesize $y_1^2$};
		
	%%%%				
	\draw[decoration={brace, mirror, raise=4}, decorate,semithick] (3,0) -- (3,1) node [pos=0.5,anchor=west,xshift=5] {\footnotesize $x_1^2$};	
	\draw[decoration={brace, mirror, raise=18}, decorate,semithick] (3,0) -- (3,2) node [pos=0.5,anchor=west,xshift=19] {\footnotesize $\sum\limits_{j=1}^i x_j^2$};		
	%%%%		
	\draw[decoration={brace, mirror, raise=4}, decorate,semithick] (5,0) -- (5,1.66) node [pos=0.5,anchor=west,xshift=5] {\footnotesize $y_1^2$};	
	\draw[decoration={brace, mirror, raise=18}, decorate,semithick] (5,0) -- (5,3.33) node [pos=0.5,anchor=west,xshift=19] {\footnotesize $\sum\limits_{j=1}^i y_j^2$};	
	%%%%
		\draw[decoration={brace, mirror, raise=46}, decorate,semithick,-] (5,0) -- (5,5) node [pos=0.5,anchor=west,xshift=47] {\footnotesize $b$};
	%%%%
					
\end{tikzpicture}

